DYAD: A Descriptive Yet Abjuring Density efficient approximation to linear neural network layers

We devise, implement and performance-asses DYAD, a layer which can serve as a faster and more memory-efficient approximate replacement for linear layers, (nn.Linear() in Pytorch). These layers appear in common subcomponents, such as in the ff module of Transformers. DYAD is based on a bespoke near-sparse matrix structure which approximates the dense "weight" matrix W that matrix-multiplies the input in the typical realization of such a layer, a.k.a DENSE. Our alternative near-sparse matrix structure is decomposable to a sum of 2 matrices permutable to a block-sparse counterpart. These can be represented as 3D tensors, which in unison allow a faster execution of matrix multiplication with the mini-batched input matrix X compared to DENSE (O(rows(W ) x cols(W )) --> O( rows(W ) x cols(W ) # of blocks )). As the crux of our experiments, we pretrain both DYAD and DENSE variants of 2 sizes of the OPT arch and 1 size of the Pythia arch, including at different token scales of the babyLM benchmark. We find DYAD to be competitive (>= 90%) of DENSE performance on zero-shot (e.g. BLIMP), few-shot (OPENLM) and finetuning (GLUE) benchmarks, while being >=7-15% faster to train on-GPU even at 125m scale, besides surfacing larger speedups at increasing scale and model width.

==> OriginalTemplate.tex <==
% partial rewrite of the LaTeX2e package for submissions to the
% Conference on Neural Information Processing Systems (NeurIPS):
%
% - uses more LaTeX conventions
% - line numbers at submission time replaced with aligned numbers from
%   lineno package
% - \nipsfinalcopy replaced with [final] package option
% - automatically loads times package for authors
% - loads natbib automatically; this can be suppressed with the
%   [nonatbib] package option
% - adds foot line to first page identifying the conference
% - adds preprint option for submission to e.g. arXiv
% - conference acronym modified
%
% Roman Garnett (garnett@wustl.edu) and the many authors of
% nips15submit_e.sty, including MK and drstrip@sandia
%
% last revision: March 2023

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{neurips_2023}[2023/03/31 NeurIPS 2023 submission/camera-ready style file]

% declare final option, which creates camera-ready copy
\newif\if@neuripsfinal\@neuripsfinalfalse
\DeclareOption{final}{
  \@neuripsfinaltrue
}

% declare nonatbib option, which does not load natbib in case of
% package clash (users can pass options to natbib via
% \PassOptionsToPackage)
\newif\if@natbib\@natbibtrue
\DeclareOption{nonatbib}{
  \@natbibfalse
}

% declare preprint option, which creates a preprint version ready for
% upload to, e.g., arXiv
\newif\if@preprint\@preprintfalse
\DeclareOption{preprint}{
  \@preprinttrue
}

\ProcessOptions\relax

% determine whether this is an anonymized submission
\newif\if@submission\@submissiontrue
\if@neuripsfinal\@submissionfalse\fi
\if@preprint\@submissionfalse\fi

% fonts
\renewcommand{\rmdefault}{ptm}
\renewcommand{\sfdefault}{phv}

% change this every year for notice string at bottom
\newcommand{\@neuripsordinal}{37th}
\newcommand{\@neuripsyear}{2023}
\newcommand{\@neuripslocation}{New Orleans}

% acknowledgments
\usepackage{environ}
\newcommand{\acksection}{\section*{Acknowledgments and Disclosure of Funding}}
\NewEnviron{ack}{%
  \acksection
  \BODY
}


% load natbib unless told otherwise
\if@natbib
  \RequirePackage{natbib}
\fi

% set page geometry
\usepackage[verbose=true,letterpaper]{geometry}
\AtBeginDocument{
  \newgeometry{
    textheight=9in,
    textwidth=5.5in,
    top=1in,
    headheight=12pt,
    headsep=25pt,
    footskip=30pt
  }
  \@ifpackageloaded{fullpage}
    {\PackageWarning{neurips_2023}{fullpage package not allowed! Overwriting formatting.}}
    {}
}

\widowpenalty=10000
\clubpenalty=10000
\flushbottom
\sloppy


% font sizes with reduced leading
\renewcommand{\normalsize}{%
  \@setfontsize\normalsize\@xpt\@xipt
  \abovedisplayskip      7\p@ \@plus 2\p@ \@minus 5\p@
  \abovedisplayshortskip \z@ \@plus 3\p@
  \belowdisplayskip      \abovedisplayskip
  \belowdisplayshortskip 4\p@ \@plus 3\p@ \@minus 3\p@
}
\normalsize
\renewcommand{\small}{%
  \@setfontsize\small\@ixpt\@xpt
  \abovedisplayskip      6\p@ \@plus 1.5\p@ \@minus 4\p@
  \abovedisplayshortskip \z@  \@plus 2\p@
  \belowdisplayskip      \abovedisplayskip
  \belowdisplayshortskip 3\p@ \@plus 2\p@   \@minus 2\p@
}
\renewcommand{\footnotesize}{\@setfontsize\footnotesize\@ixpt\@xpt}
\renewcommand{\scriptsize}{\@setfontsize\scriptsize\@viipt\@viiipt}
\renewcommand{\tiny}{\@setfontsize\tiny\@vipt\@viipt}
\renewcommand{\large}{\@setfontsize\large\@xiipt{14}}
\renewcommand{\Large}{\@setfontsize\Large\@xivpt{16}}
\renewcommand{\LARGE}{\@setfontsize\LARGE\@xviipt{20}}
\renewcommand{\huge}{\@setfontsize\huge\@xxpt{23}}
\renewcommand{\Huge}{\@setfontsize\Huge\@xxvpt{28}}

% sections with less space
\providecommand{\section}{}
\renewcommand{\section}{%
  \@startsection{section}{1}{\z@}%
                {-2.0ex \@plus -0.5ex \@minus -0.2ex}%
                { 1.5ex \@plus  0.3ex \@minus  0.2ex}%
                {\large\bf\raggedright}%
}
\providecommand{\subsection}{}
\renewcommand{\subsection}{%
  \@startsection{subsection}{2}{\z@}%
                {-1.8ex \@plus -0.5ex \@minus -0.2ex}%
                { 0.8ex \@plus  0.2ex}%
                {\normalsize\bf\raggedright}%
}
\providecommand{\subsubsection}{}
\renewcommand{\subsubsection}{%
  \@startsection{subsubsection}{3}{\z@}%
                {-1.5ex \@plus -0.5ex \@minus -0.2ex}%
                { 0.5ex \@plus  0.2ex}%
                {\normalsize\bf\raggedright}%
}
\providecommand{\paragraph}{}
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}{\z@}%
                {1.5ex \@plus 0.5ex \@minus 0.2ex}%
                {-1em}%
                {\normalsize\bf}%
}
\providecommand{\subparagraph}{}
\renewcommand{\subparagraph}{%
  \@startsection{subparagraph}{5}{\z@}%
                {1.5ex \@plus 0.5ex \@minus 0.2ex}%
                {-1em}%
                {\normalsize\bf}%
}
\providecommand{\subsubsubsection}{}
\renewcommand{\subsubsubsection}{%
  \vskip5pt{\noindent\normalsize\rm\raggedright}%
}

% float placement
\renewcommand{\topfraction      }{0.85}
\renewcommand{\bottomfraction   }{0.4}
\renewcommand{\textfraction     }{0.1}
\renewcommand{\floatpagefraction}{0.7}

\newlength{\@neuripsabovecaptionskip}\setlength{\@neuripsabovecaptionskip}{7\p@}
\newlength{\@neuripsbelowcaptionskip}\setlength{\@neuripsbelowcaptionskip}{\z@}

\setlength{\abovecaptionskip}{\@neuripsabovecaptionskip}
\setlength{\belowcaptionskip}{\@neuripsbelowcaptionskip}

% swap above/belowcaptionskip lengths for tables
\renewenvironment{table}
  {\setlength{\abovecaptionskip}{\@neuripsbelowcaptionskip}%
   \setlength{\belowcaptionskip}{\@neuripsabovecaptionskip}%
   \@float{table}}
  {\end@float}

% footnote formatting
\setlength{\footnotesep }{6.65\p@}
\setlength{\skip\footins}{9\p@ \@plus 4\p@ \@minus 2\p@}
\renewcommand{\footnoterule}{\kern-3\p@ \hrule width 12pc \kern 2.6\p@}
\setcounter{footnote}{0}

% paragraph formatting
\setlength{\parindent}{\z@}
\setlength{\parskip  }{5.5\p@}

% list formatting
\setlength{\topsep       }{4\p@ \@plus 1\p@   \@minus 2\p@}
\setlength{\partopsep    }{1\p@ \@plus 0.5\p@ \@minus 0.5\p@}
\setlength{\itemsep      }{2\p@ \@plus 1\p@   \@minus 0.5\p@}
\setlength{\parsep       }{2\p@ \@plus 1\p@   \@minus 0.5\p@}
\setlength{\leftmargin   }{3pc}
\setlength{\leftmargini  }{\leftmargin}
\setlength{\leftmarginii }{2em}
\setlength{\leftmarginiii}{1.5em}
\setlength{\leftmarginiv }{1.0em}
\setlength{\leftmarginv  }{0.5em}
\def\@listi  {\leftmargin\leftmargini}
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep  2\p@ \@plus 1\p@    \@minus 0.5\p@
              \parsep  1\p@ \@plus 0.5\p@ \@minus 0.5\p@
              \itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    1\p@ \@plus 0.5\p@ \@minus 0.5\p@
              \parsep    \z@
              \partopsep 0.5\p@ \@plus 0\p@ \@minus 0.5\p@
              \itemsep \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}

% create title
\providecommand{\maketitle}{}
\renewcommand{\maketitle}{%
  \par
  \begingroup
    \renewcommand{\thefootnote}{\fnsymbol{footnote}}
    % for perfect author name centering
    \renewcommand{\@makefnmark}{\hbox to \z@{$^{\@thefnmark}$\hss}}
    % The footnote-mark was overlapping the footnote-text,
    % added the following to fix this problem               (MK)
    \long\def\@makefntext##1{%
      \parindent 1em\noindent
      \hbox to 1.8em{\hss $\m@th ^{\@thefnmark}$}##1
    }
    \thispagestyle{empty}
    \@maketitle
    \@thanks
    \@notice
  \endgroup
  \let\maketitle\relax
  \let\thanks\relax
}

% rules for title box at top of first page
\newcommand{\@toptitlebar}{
  \hrule height 4\p@
  \vskip 0.25in
  \vskip -\parskip%
}
\newcommand{\@bottomtitlebar}{
  \vskip 0.29in
  \vskip -\parskip
  \hrule height 1\p@
  \vskip 0.09in%
}

% create title (includes both anonymized and non-anonymized versions)
\providecommand{\@maketitle}{}
\renewcommand{\@maketitle}{%
  \vbox{%
    \hsize\textwidth
    \linewidth\hsize
    \vskip 0.1in
    \@toptitlebar
    \centering
    {\LARGE\bf \@title\par}
    \@bottomtitlebar
    \if@submission
      \begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}
        Anonymous Author(s) \\
        Affiliation \\
        Address \\
        \texttt{email} \\
      \end{tabular}%
    \else
      \def\And{%
        \end{tabular}\hfil\linebreak[0]\hfil%
        \begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}\ignorespaces%
      }
      \def\AND{%
        \end{tabular}\hfil\linebreak[4]\hfil%
        \begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}\ignorespaces%
      }
      \begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}\@author\end{tabular}%
    \fi
    \vskip 0.3in \@minus 0.1in
  }
}

% add conference notice to bottom of first page
\newcommand{\ftype@noticebox}{8}
\newcommand{\@notice}{%
  % give a bit of extra room back to authors on first page
  \enlargethispage{2\baselineskip}%
  \@float{noticebox}[b]%
    \footnotesize\@noticestring%
  \end@float%
}

% abstract styling
\renewenvironment{abstract}%
{%
  \vskip 0.075in%
  \centerline%
  {\large\bf Abstract}%
  \vspace{0.5ex}%
  \begin{quote}%
}
{
  \par%
  \end{quote}%
  \vskip 1ex%
}

% handle tweaks for camera-ready copy vs. submission copy
\if@preprint
  \newcommand{\@noticestring}{%
    Preprint. Under review.%
  }
\else
  \if@neuripsfinal
    \newcommand{\@noticestring}{%
      \@neuripsordinal\/ Conference on Neural Information Processing Systems
      (NeurIPS \@neuripsyear).%, \@neuripslocation.%
    }
  \else
    \newcommand{\@noticestring}{%
      Submitted to \@neuripsordinal\/ Conference on Neural Information
      Processing Systems (NeurIPS \@neuripsyear). Do not distribute.%
    }

    % hide the acknowledgements
    \NewEnviron{hide}{}
    \let\ack\hide
    \let\endack\endhide

    % line numbers for submission
    \RequirePackage{lineno}
    \linenumbers

    % fix incompatibilities between lineno and amsmath, if required, by
    % transparently wrapping linenomath environments around amsmath
    % environments
    \AtBeginDocument{%
      \@ifpackageloaded{amsmath}{%
        \newcommand*\patchAmsMathEnvironmentForLineno[1]{%
          \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
          \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
          \renewenvironment{#1}%
                          {\linenomath\csname old#1\endcsname}%
                          {\csname oldend#1\endcsname\endlinenomath}%
        }%
        \newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
          \patchAmsMathEnvironmentForLineno{#1}%
          \patchAmsMathEnvironmentForLineno{#1*}%
        }%
        \patchBothAmsMathEnvironmentsForLineno{equation}%
        \patchBothAmsMathEnvironmentsForLineno{align}%
        \patchBothAmsMathEnvironmentsForLineno{flalign}%
        \patchBothAmsMathEnvironmentsForLineno{alignat}%
        \patchBothAmsMathEnvironmentsForLineno{gather}%
        \patchBothAmsMathEnvironmentsForLineno{multline}%
      }
      {}
    }
  \fi
\fi


\endinput


==> sections/formulationOld.tex <==
%\varun{Below is just to show example footnote and use of custom symbols etc}
%We curate a dataset called {\DatasetName} of 511 personifications, with 236 coming from a publicly available open-sourced list\footnote{\url{https://www.kaggle.com/datasets/varchitalalwani/figure-of-speech}} and 275 manually-filtered personifications extracted from the Deja dataset . The Deja dataset is an image-captioning dataset containing a ``figurative'' subset of size 6000, of which $4.1\%$ of the captions are labelled as personifications. We extract these personifications and combine them with our existing list to form the final {\DatasetName} dataset.
\subsection{Linear Layer}
A Linear layer is the basic building block of all neural networks, represented in pytorch by \verb|nn.Linear()|. It maps input $X$ to output $Y$ via a dense matrix multiplication with weight matrix $W$, given by the equation $Y = G_{Linear}(X) = WX+b$. Here, $W$ is a matrix of shape $f_{out} \times f_{in}$ where $f_{out}$ and $f_{in}$ represent the no. of output \& input features. $Y$, $X$ and the bias $b$ have shapes $f_{out} \times n_{batch}$, ${f}_{in} \times n_{batch}$ and $f_{out} \times 1$. Frameworks like pytorch pose the shape of $X$ and $Y$ as $n_{batch} \times f_{in}$ and $n_{batch} \times f_{out}$ but here we adhere to the former convention.

\subsection{\textsc{\LayerGroupName} : Definition and Properties}
Here, we introduce a family of sparse layers named \textsc{\LayerGroupName} that can serve as an approximate replacement for the dense linear layer. \textsc{\LayerGroupName} has 3 variants called \textsc{\LayerVariantNameI}, \textsc{\LayerVariantNameII} and \textsc{\LayerVariantNameIII}. The initials stand for Input Transpose, Output Transpose and Double Transpose. They are named such because transpose operations on either the input or output enables to compute their outputs efficiently. We describe \textsc{\LayerVariantNameI} here but defer describing the other two to the appendix.
\begin{comment}
\begin{figure*}
    \centering
    \includegraphics[width=0.26\textwidth]{sections/Figures/Dyad - Input Transpose.png}
    \caption{Dyad Weight Matrix}
    \label{fig:dyad-input-transpose}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[scale=0.23]{sections/Figures/Dyad - IT Componenets.png}
    \caption{Dyad Weight Matrix Components}
    \label{fig:dyad-input-transpose-componenets}
\end{figure*}
\end{comment}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.25\textwidth,frame]{sections/Figures/Dyad - Input Transpose.png}
    %\subcaption{Dyad Weight Matrix}
    %\label{fig:dyad-input-transpose}
    \includegraphics[width=0.52\textwidth,frame]{sections/Figures/Dyad - IT Componenets.png}
    %\subcaption{Dyad Weight Matrix Components}
    %\label{fig:dyad-input-transpose-componenets}
    \caption{\footnotesize Dyad Weight Matrix [L] vs its Components [R], {\DyadComponentIShorthand} \& {\DyadComponentIIShorthand}. Green is $\neq 0$. } \label{fig:dyad-input-transpose-components}
\vspace{-3mm}
\end{figure*}
%\subsubsection{\textsc{\LayerGroupName} Definition}
\textsc{\LayerGroupName} is a linear layer with a sparse weight matrix having shape shown in Fig \ref{fig:dyad-input-transpose-components}. The output of this layer can be calculated using $G_{Linear}$. However, this won't lead to any efficiency gain compared to the linear layer. We can split the \textsc{\LayerGroupName} matrix into 2 components as shown in Fig \ref{fig:dyad-input-transpose-components}. These components share some non-zero elements but their sum's representational power would be identical to the \textsc{\LayerGroupName} matrix. We call the first component the \textit{\DyadComponentI} ({\DyadComponentIShorthand}) and the second one the \textit{\DyadComponentII} ({\DyadComponentIIShorthand}). The ability to split \textsc{\LayerGroupName} into 2 components is what inspires its name. A \textsc{\LayerGroupName} matrix can be defined using 3 parameters, \textsc{\DyadDim}, \textsc{\DimIn} and \textsc{\DimOut}. \textsc{\DimOut} $\times$ \textsc{\DimIn} is the size of each submatrix in \textit{\DyadComponentIShorthand} and \textsc{\DyadDim} represents the no. of submatrixes in each component. Thus, all the figures for \textsc{\LayerGroupName} shown here have $n_{dyad}=n_{in}=n_{out}=4$. With the 2 components of \textsc{\LayerGroupName} split up, we can write its layer output as in Eq \ref{dyadFullEq}.
% We can see these components annotated in Fig \ref{fig:block-diag-matrix}. 
%\begin{figure*}
%    \centering
%    \includegraphics[width=0.49\textwidth]{sections/Figures/Dyad - Annotated.png}
%    \caption{Block Diagonal Component.}
%    \label{fig:block-diag-matrix}
%\end{figure*}
\begin{align}
    Y &= W_1X + W_2X + b \label{dyadFullEq}
\end{align}
Naively implementing this as in Eq \ref{dyadFullEq}, will be as expensive as its dense counterpart. To exploit the joint properties of sparsity and block structure in these 2 components, we need to transform $W_1X$ and  $W_2X$ to an equivalent sequence of 3D tensor operands and operations.

Hereforth, we ease representing 3D tensors in our equations by overloading pytorch tensor operators.

\subsubsection{Efficient Computation of {\DyadComponentIShorthand}}
{\DyadComponentIShorthand} as in Fig \ref{fig:dyad-input-transpose-components} is of size (\textsc{\DyadDim}$\times$\textsc{\DimOut} , \textsc{\DyadDim}$\times$\textsc{\DimIn}). We can store this weight matrix efficiently as a 3D tensor, $W_1^{'}$, of shape (\textsc{\DyadDim},\textsc{\DimOut},\textsc{\DimIn}). This is a factor of \textsc{\DyadDim} times smaller. All elements of the 3D tensor map to the weight matrix as shown in Eq \ref{DyadMap}.
{\small\begin{align}
    W_1^{'}[i,j,k] &= W_1[i*{{n}_{out}}+j,i*{{n}_{in}}+k] \label{DyadMap}
\end{align}}%
All the elements of $W_1$ outside of the ones assigned in Eq \ref{DyadMap} will be zero. From Fig \ref{fig:dyad-input-transpose-components} we can see that for any output index in the range $i \times {{n}_{out}}$ to $(i + 1) \times {{n}_{out}}$ only depends on input indices in the range $i \times {{n}_{in}}$ to $(i + 1) \times {{n}_{in}}$ where $i \in$ $[0,$\textsc{\DyadDim}$)$. This shows that each pair of input and output dimensions can be calculated individually using a matrix multiplication for each block and thus the whole output can be calculated using a batched matrix multiplication as shown in Eq \ref{diagBMM} after the input has been also converted to a 3D tensor as shown in Eq \ref{diagReshape}.
{\small\begin{align}
    X_1^{'} &= X.reshape({{n}_{dyad}},{{n}_{in}},n_{batch}) \label{diagReshape}\\
    Y_1 &= W_1^{'}.bmm(X_1^{'}).reshape({{n}_{dyad}} \times {{n}_{out}},{n}_{batch}) \label{diagBMM}
\end{align}}%
The value of $Y_1$ here is the same as $W_1X$ in Eq \ref{dyadFullEq} but cost of computing it will be $O({{n}_{dyad}} \times {{n}_{out}} \times {{n}_{in}})$ instead of $O({n}_{dyad}^{2} \times {{n}_{out}} \times {{n}_{in}})$ which is $O({{n}_{dyad}})$ times faster.

\subsubsection{Efficient Computation of {\DyadComponentIIShorthand}}
The matrix multiplication for {\DyadComponentIIShorthand}, i.e. $W_2X$ can be converted to a form similar to {\DyadComponentIShorthand} by permuting the columns of $W_2$. A permutation matrix, $P$ is a square matrix which has exactly one element along each row and each column as one and the rest have a value of zero. Pre-multiplying by a permutation matrix, i.e of the form $PA$, permutes the rows of matrix $A$, while post-multiplying by a permutation matrix, i.e. of the form $AP$ permutes the columns of matrix $A$. So if we post multiply, $W_2$ by an appropriate permutation matrix which has the form as shown in Eq \ref{PermuteEq}, we will end up with a matrix similar in structure to {\DyadComponentIShorthand}. 
{\footnotesize\begin{align}
    P(i,j) &= 
\begin{cases}
    1,& \text{if } j={{n}_{dyad}}*(i\%{{n}_{in}}) + i//{{n}_{in}} \label{PermuteEq} \\
    0,              & \text{otherwise}
\end{cases}
\end{align}}%
\begin{wrapfigure}{l}{0.34\textwidth}
%\begin{figure*}
    %\centering
    \includegraphics[width=0.99\linewidth]{sections/Figures/Permutation Matrix.png}
    \caption{Permutation Matrix for \DyadComponentIIShorthand}
    \label{fig:permutation-matrix}
%\end{figure*}
\end{wrapfigure}
\begin{comment}
\begin{wrapfigure}{l}{0.25\textwidth}
\includegraphics[width=0.9\linewidth]{overleaf-logo} 
\caption{Caption1}
\label{fig:wrapfig}
\end{wrapfigure}
\end{comment}
For the Dyad matrix with {\DyadDim}, {\DimIn} and {\DimOut} of 4 each, this permutation matrix is shown in Fig \ref{fig:permutation-matrix}. As Permutation matrices are orthonormal, $P^{-1} = P^{T}$ where $P^{T}$ is another Permutation matrix \cite{wiki-matrix-perm-properties}. 
{\footnotesize\begin{align}
    Y_2 = W_2X = W_2(PP^{T})X = (W_2P)(P^{T}X) \label{permuteComp}
\end{align}}%
Using the othonormal property of permutation matrixes we can write $W_2X$ as shown in Eq \ref{permuteComp}. Here, $Y_2$ is the output of {\DyadComponentIIShorthand}. Let $W_2^{P} = W_2P$ and $X_2^{P} = P^{T}X$. Since, $W_2^{P}$ has the same structure as the weight matrix for {\DyadComponentIShorthand}, we can also store it as a 3D tensor of shape ${{n}_{dyad}} \times {{n}_{out}} \times {{n}_{in}}$. Hence, as in the case before this leads to a reduction in memory size of $O({{n}_{dyad}})$ when compared to $W_2$.

Calculating $P^{T}X$ naively in order to get $X_2^{P}$ for every input can end up being as expensive as the computation cost of a linear layer. However, the specific pattern of the permutation allows us to calculate $X_2^{P}$ by simplying transposing a 3D view of $X$. This can be seen from Eq \ref{PermuteEq} where within a multiple of {\DimIn} for every increment of $i$, $j$ increases by {\DyadDim} while for every $i + {{n}_{in}}$ increment j only increase by 1. Thus, $i$ can be thought of as the 1D index of a flattened 2D matrix of shape ${{n}_{dyad}} \times {{n}_{in}}$ with stride $(1, {{n}_{dyad}})$. Hence, permuting and inverting the permutation can be done by just transposing this 2D matrix i.e. going from shape ${{n}_{dyad}} \times {{n}_{in}}$ to ${{n}_{in}} \times {{n}_{dyad}}$ and from stride $(1, {{n}_{dyad}})$ to stride $({{n}_{dyad}},1)$ and vice versa. Calculating $X_2^{P}$ this way from $X$ is shown in Eq \ref{Xpermute}.
{\footnotesize\begin{align}
    X_2^{P} &= X.reshape({{n}_{in}},{{n}_{dyad}},-1).transpose(0,1).reshape(-1, {n}_{batch}) \label{Xpermute} \\
    X_2^{'} &= X_2^{P}.reshape({{n}_{dyad}},{{n}_{in}},{n}_{batch}) \label{X3d} \\
    X_2^{'} &= X.reshape({{n}_{in}},{{n}_{dyad}},{n}_{batch}).transpose(0,1) \label{Xcomp2Eq}
\end{align}}%
Now as in the case of {\DyadComponentIShorthand} we need the activations as a 3D tensor to do the calculations efficiently. So we need to reshape $X_2^{P}$ as shown in Eq \ref{X3d} to get $X_2^{'}$. $X_2^{'}$ is the actual activation input for the batched matrix multiplication. We can combine Eq \ref{Xpermute} and \ref{X3d} to cancel the reshape as shown in \ref{Xcomp2Eq}. Eq \ref{Xcomp2Eq} is basically free and involves just changing some metadata related to the strides of the dimensions. The actual data of the tensor need not be touched here. 
\begin{align}
    Y_2 &= W_2^{'}.bmm(X_2^{'}).reshape({{n}_{dyad}} \times {{n}_{out}}, {n}_{batch}) \label{comp2eq}
\end{align}
Thus, {\DyadComponentIIShorthand} calculation can be performed as shown in Eq \ref{comp2eq}. The cost of computation here is again same as that of the previous case with complexity $O({{n}_{dyad}} \times {{n}_{out}} \times {{n}_{in}})$ and is faster by a factor of $O({{n}_{dyad}})$ when compared with multiplying with $W_2$. The {\LayerGroupName} layer can be written relatively efficiently in pytorch, as shown in Appendix \S 6.1. In Appendix \S 6.2.2, we discuss some thoughts about the representational power of \textsc{\LayerGroupName}. 


==> sections/related_work.tex <==
In this work, we focus specifically on the linear layers that are a building block in feedforward and other blocks/components/meta-layers. 

==> sections/todo.tex <==
Rounding in tables
Combining table with minipage
Making tables more beautiful with booktabs
Adding histogram for mean values
